The METRIC-framework for assessing data quality for trustworthy AI in medicine: a systematic review

The adoption of machine learning (ML) and, more specifically, deep learning (DL) applications into all major areas of our lives is underway. The development of trustworthy AI is especially important in medicine due to the large implications for patients' lives. While trustworthiness concerns various aspects including ethical, technical and privacy requirements, we focus on the importance of data quality (training/test) in DL. Since data quality dictates the behaviour of ML products, evaluating data quality will play a key part in the regulatory approval of medical AI products. We perform a systematic review following PRISMA guidelines using the databases PubMed and ACM Digital Library. We identify 2362 studies, out of which 62 records fulfil our eligibility criteria. From this literature, we synthesise the existing knowledge on data quality frameworks and combine it with the perspective of ML applications in medicine. As a result, we propose the METRIC-framework, a specialised data quality framework for medical training data comprising 15 awareness dimensions, along which developers of medical ML applications should investigate a dataset. This knowledge helps to reduce biases as a major source of unfairness, increase robustness, facilitate interpretability and thus lays the foundation for trustworthy AI in medicine. Incorporating such systematic assessment of medical datasets into regulatory approval processes has the potential to accelerate the approval of ML products and builds the basis for new standards.

==> tables/definitions.tex <==
\begin{tabular}{| p{3.7cm} | p{3.3cm} | p{3.5cm} |  p{3.5cm} |}
\hline
Major category & DQ dimension & DQ subdimension & references \\
\end{tabular}
\begin{tabular}{| p{3.7cm} | p{3.3cm} | p{3.5cm} |  p{3.5cm} |}
\hline
\rule{0pt}{10pt} \bf representativeness&&&\footnotesize  \\
\hline
&\raggedright representativeness of population& \ &\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&relevance&\footnotesize  \\
\cdashline{3-4}[0.5pt/2.5pt]
&&sufficiency&\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&variety of data and data sources&\footnotesize  \\
\cdashline{3-4}[0.5pt/2.5pt]
&&flexibility&\footnotesize \\
\cdashline{2-4}
&\raggedright representativeness for technology& \ &\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&class balance &\footnotesize \\
\hline
\end{tabular}
\begin{tabular}{| p{3.7cm} | p{3.3cm} | p{3.5cm} |  p{3.5cm} |}
\hline
\rule{0pt}{10pt} \bf informativeness&&&\footnotesize \\
\hline
&\raggedright amount of data& \ &\footnotesize  \\
\cdashline{3-4}[0.5pt/2.5pt]
&&dataset size&\footnotesize  \\
\cdashline{3-4}[0.5pt/2.5pt]
&&granularity&\footnotesize  \\
\cdashline{2-4}
&\raggedright missingness& \ &\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&completeness&\footnotesize  \\
\cdashline{3-4}[0.5pt/2.5pt]
&&informative missingness&\footnotesize \\
\cdashline{2-4}
&\raggedright added value& \ &\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&usefulness&\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&feature importance&\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&understandability&\footnotesize  \\
\cdashline{2-4}
&\raggedright redundancy& \ &\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&uniqueness&\footnotesize  \\
\cdashline{3-4}[0.5pt/2.5pt]
&&conciseness&\footnotesize \\
\hline
\end{tabular}
\begin{tabular}{| p{3.7cm} | p{3.3cm} | p{3.5cm} |  p{3.5cm} |}
\hline
\rule{0pt}{10pt} \bf reliability&&&\footnotesize  \\
\hline
&\raggedright lineage& \ &\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&traceability&\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&modification&\footnotesize \\
\cdashline{2-4}
&\raggedright measurement uncertainty& \ &\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&accuracy&\footnotesize  \\
\cdashline{3-4}[0.5pt/2.5pt]
&&precision &\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&outlier&\footnotesize  \\
\cdashline{2-4}
&\raggedright target uncertainty& \ &\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&noisy labels&\footnotesize \\
\cdashline{2-4}
&\raggedright credibility& \ &\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&plausibility&\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&believability&\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&source legitimacy&\footnotesize \\
\hline
\end{tabular}
\begin{tabular}{| p{3.7cm} | p{3.3cm} | p{3.5cm} |  p{3.5cm} |}
\hline
\rule{0pt}{10pt} \bf consistency&&&\footnotesize  \\
\hline
&\raggedright syntactic consistency& \ &\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&internal syntactic consistency&\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&external syntactic consistency&\footnotesize \\
\cdashline{2-4}
&\raggedright semantic consistency& \ &\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&intra-dataset sem. consistency&\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&inter-dataset sem. consistency&\footnotesize \\
\cdashline{2-4}
&\raggedright distribution consistency& \ &\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&homogeneity&\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&distribution drift&\footnotesize \\
\hline
\end{tabular}
\begin{tabular}{| p{3.7cm} | p{3.3cm} | p{3.5cm} |  p{3.5cm} |}
\hline
\rule{0pt}{10pt} \bf timeliness&&&\footnotesize \\
\hline
&\raggedright age& \ &\footnotesize \\
\cdashline{2-4}
&\raggedright currency& \ &\footnotesize \\
\hline
\end{tabular}
\begin{tabular}{| p{3.7cm} | p{3.3cm} | p{3.7cm} |  p{3.5cm} |}
\hline
\rule{0pt}{10pt} \bf eligibility&&&\footnotesize \\
\hline
&\raggedright documentation& \ &\footnotesize \\
\cdashline{2-4}
&\raggedright data schema& \ &\footnotesize \\
\cdashline{2-4}
&\raggedright privacy& \ &\footnotesize \\
\cdashline{2-4}
&\raggedright security& \ &\footnotesize \\
\cdashline{2-4}
&\raggedright FAIR principles& \ &\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&accessibility&\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&interoperability&\footnotesize \\
\cdashline{3-4}[0.5pt/2.5pt]
&&reusability&\footnotesize \\
\hline
\end{tabular}\label{tab:fettetabelle}
